PTaRL: Prototype-based Tabular Representation Learning via Space Calibration

Tabular data have been playing a mostly important role in diverse real-world fields, such as healthcare, engineering, finance, etc. With the recent success of deep learning, many tabular machine learning (ML) methods based on deep networks (e.g., Transformer, ResNet) have achieved competitive performance on tabular benchmarks. However, existing deep tabular ML methods suffer from the representation entanglement and localization, which largely hinders their prediction performance and leads to performance inconsistency on tabular tasks. To overcome these problems, we explore a novel direction of applying prototype learning for tabular ML and propose a prototype-based tabular representation learning framework, PTaRL, for tabular prediction tasks. The core idea of PTaRL is to construct prototype-based projection space (P-Space) and learn the disentangled representation around global data prototypes. Specifically, PTaRL mainly involves two stages: (i) Prototype Generation, that constructs global prototypes as the basis vectors of P-Space for representation, and (ii) Prototype Projection, that projects the data samples into P-Space and keeps the core global data information via Optimal Transport. Then, to further acquire the disentangled representations, we constrain PTaRL with two strategies: (i) to diversify the coordinates towards global prototypes of different representations within P-Space, we bring up a diversification constraint for representation calibration; (ii) to avoid prototype entanglement in P-Space, we introduce a matrix orthogonalization constraint to ensure the independence of global prototypes. Finally, we conduct extensive experiments in PTaRL coupled with state-of-the-art deep tabular ML models on various tabular benchmarks and the results have shown our consistent superiority.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/comment_AC.tex <==
\section{Rebuttal}
Dear AC, 

We appreciate all the reviewers and area chairs for the dedicated efforts invested in reviewing our paper. In response to the additional concern raised by Reviewer 7NUi, we have revised our workflow to make Line 18 in Algorithm 1 more understandable. 
The details of Line 18 are as follows: Update $\mathcal{B}, \theta_f, \theta_h, \gamma$ by minimizing $\mathcal{O} = \mathcal{L}_{task} + \mathcal{L}_{projecting} + \mathcal{L}_{diversifying} + \mathcal{L}_{orthogonalization}$ through gradient descent. We also provide sensitivity analysis about the loss weights in Appendix A.6. Other concerns raised by the reviewers have been addressed before. After the informative discussions with the reviewers, we are delighted to see that the ratings have been increased to 8, 8, 8.

In this work, we first investigate the learned patterns of deep tabular machine learning models and identify two inherent characteristic hindering prediction: (i) representation entanglement and representation localization. To overcome these challenges, we then explore the direction of applying prototype learning for deep tabular machine learning. The proposed representation learning pipeline PTaRL can be integrated into various deep tabular models. The extensive experiments on various tabular benchmarks have shown our consistent superiority. The novelty and contribution have been proved by the reviewers.

% This work embodies the efforts of all the authors, where the first author have made a lot of efforts as the first year doctoral student. 
We aspire for our work to contribute to the advancement of deep learning in tabular data and hope that it captures the attention of researchers in the field. 

Best regards,

The authors


==> sections/comment_AC_short.tex <==
\section{Rebuttal}
Dear AC, 

We appreciate your and all the reviewers' dedicated efforts invested in reviewing our paper very much. Initially, we received very positive ratings from the reviewers. After the informative discussions with the reviewers, we are delighted to see that the ratings have been increased to 8, 8, 8. Although the ratings are yet to be finalized, the recognition of our paper's contributions by the reviewers is already very encouraging and the useful comments we have received will sure make our paper stronger.

In addition to the technical novelty and contributions, our paper is an excellent example of international collaborations between academia and industry. More importantly, this research is led by the first author who just started their research career as a first-year PhD student. We humbly believe that our paper might possibly be a candidate of representing the breadth of excellent research being conducted by the ICLR community. If appropriate, your recommendation of the acceptance or even nomination for an award
of our paper would be a great encouragement to us (especially the first author, a next-generation researcher). Thanks a lot.

Best regards,
The authors


==> sections/method.tex <==
\section{Proposed Method: \method}

% \subsection{The inherent limitations of deep networks for tabular domain.}
\subsection{Motivation}
\label{sec:entanglement details} 
In the context of tabular data, the intrinsic heterogeneity presents a challenge for achieving satisfactory performance using deep models. 
As shown in the Section~\ref{sec:introduction}, the latent representations learned by the FT-Transformer \citep{gorishniy2021revisiting}, one of the SOTA encoder networks, on a binary classification data Adult are entangled.
To validate whether it is caused by the limitation of model capacity, we gradually increase the FT-Transformer layers and visualize the corresponding latent representation. As shown in the first row of Fig.~\ref{fig:source}, with a sequential increase in the number of model layers, we could observe the entanglement phenomenon has not be mitigated while gradually augmenting the model capacity.
In addition, our empirical observations indicate that this phenomenon also exists for other deep networks and we recognize that the representation entanglement problem is the inherent limitation of deep networks in tabular domain.
On the other hand, the learned representations also lack global data structure information, which failed to model the shared information among the data instances.
Compared to other domain like images and texts, especially in the heterogeneous tabular domain, samples overlook the statistical information among the total dataset would drop into the localization situation.
These limitations could be solved to greatly enhance the progress in tabular deep networks researches.
Furthermore, recent researches ~\citep{gorishniy2021revisiting, shwartz2022tabular} show that different types of data may require varying types of deep networks (e.g. Transformer based and MLP based architecture). 

% and to adapt to different types of data, we propose a model-agnostic method PTaRL to universally enhance the performance of deep tabular networks.
\textcolor{red}{Move the explanation of Figure 2 to 4.2}
As shown in the second row of Fig.~\ref{fig:source}, with PTaRL, the latent space is calibrated to make the representation disentangled.



% We propose prototype-based tabular representation learning (\method), which is a learning procedure designed to enhance deep tabular network $F(\cdot;\theta)$'s representation quality, rather than being a specific model.
% Before introducing \method, we first give the definition of \textit{Prototype-based Projection Space}, which is the core of \method.
% Then we will elaborate the details of the PTaRL, which generates decoupled representation with global data.
% Furthermore, we provide two constraints for better guiding the process of PTaRL.


% -------Wei----------

% To address the aforementioned limitations of deep networks for the tabular domain in Section \ref{sec:entanglement details}, we apply prototype learning into tabular modeling and propose the prototype-based tabular representation learning (\method) framework. Note that \method, as a general representation learning pipeline, is model-agnostic such that it can be coupled with any deep tabular ML models $F(\cdot;\theta)$ to learn better tabular data representations in our redefined \textit{Prototype-based Projection Space}, which is the core of \method.
% In the following, we will elaborate on the specific learning procedure of our \method in Section \ref{sec:ptarl_main}; then, we will provide two constraints to further constraint \method for representation calibration and prototype independence in Section \ref{sec:ptarl_constraints}. 
% Before the introduction of \method, we first present the formal definition of the prototype-based projection space as follows.




% \textbf{Definition 1. Prototype-based Projection Space (P-Space).} Given a set of global prototypes $\mathcal{B} = \{\beta_k\}_{k=1}^K \in \mathbb{R}^{K\times d}$ where $K$ is the number of prototypes and $\beta_k$ is the representation of the $k$-th prototype with $d$ as the hidden dimension, we define the P-Space as a projection space consisting of the global prototypes $\mathcal{B}$ as the basis vectors for representation.
% % \textit{A projection space consists of a set of learnable global prototypes denoted as $B = \{\beta_k\}_{k=1}^K \in \mathbb{R}^{K\times d}$, where $K$ is the number of prototypes, $\beta_k$ is the representation of the $k$-th prototype and $d$ is the hidden dimension.}
% % Note that the global prototypes serve as the basis vectors of P-Space.
% For example, given a representation in P-Space with \textbf{\textit{coordinates}} denoted as $r = \{r^k\}_{k=1}^{K} \in \mathbb{R}^{K\times 1}$, each representation in P-Space can be formulated as $\sum_{k=1}^{K} r^k \beta_k$.
%Each latent representation of $F(\cdot;\theta)$ has the corresponding projected representation in P-Space.

% To handle the aforementioned inherent characteristic of deep tabular network $F(\cdot;\theta)$: (i) representation entanglement and (ii) sample localization,
% we couple \method with $F(\cdot;\theta)$ to learn \textit{decoupled representations} containing \textit{global data structure information}.
% Specifically, \method involves two stages: (i) prototype generating, that constructs global prototypes of P-Space, and (ii) representation projecting, that projects $F(\cdot;\theta)$'s representations into P-Space to capture global data structure information via optimal transport. 
% To further acquire the decoupled representations, we constraints \method with two strategies: (i) diversifying the coordinates $r$ of different samples in P-Space to avoid representation entanglement; (ii) orthogonalizing global prototypes to avoid prototype entanglement. 
% Fig.~\ref{fig:tab_framework} gives an overview of the proposed \method. 




\subsection{Prototype-based Tabular Representation Learning (\method)} \label{sec:ptarl_main}

\rr{Add overview The PTARL includes XXX, has xxxx}

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{pictures/tab_framework.png}
\caption{The \method framework.
}
\label{fig:tab_framework}
\vspace{-2em}
\end{figure}

To address the aforementioned limitations of deep networks for the tabular domain in Section \ref{sec:entanglement details}, we apply prototype learning into tabular modeling and propose the prototype-based tabular representation learning (\method) framework. Note that \method, as a general representation learning pipeline, is model-agnostic such that it can be coupled with any deep tabular ML model $F(\cdot;\theta)$ to learn better tabular data representations in our redefined \textit{Prototype-based Projection Space}, which is the core of \method.
In the following, we will elaborate on the specific learning procedure of our \method in Section \ref{sec:ptarl_main}; then, we will provide two constraints to further constraint \method for representation calibration and prototype independence in Section \ref{sec:ptarl_constraints}. 
Before the introduction of \method, we first present the formal definition of the prototype-based projection space as follows.



\hz{Need the motivation of introducing global prototypes. Why do we need to introduce global prototypes?}
\textbf{Definition 1. Prototype-based Projection Space (P-Space).} Given a set of global prototypes $\mathcal{B} = \{\beta_k\}_{k=1}^K \in \mathbb{R}^{K\times d}$ where $K$ is the number of prototypes and $\beta_k$ is the representation of the $k$-th prototype with $d$ as the hidden dimension, we define the P-Space as a projection space consisting of the global prototypes $\mathcal{B}$ as the basis vectors for representation.
% \textit{A projection space consists of a set of learnable global prototypes denoted as $B = \{\beta_k\}_{k=1}^K \in \mathbb{R}^{K\times d}$, where $K$ is the number of prototypes, $\beta_k$ is the representation of the $k$-th prototype and $d$ is the hidden dimension.}
% Note that the global prototypes serve as the basis vectors of P-Space.
For example, given a representation in P-Space with \textbf{\textit{coordinates}} denoted as $r = \{r^k\}_{k=1}^{K} \in \mathbb{R}^{K\times 1}$, each representation in P-Space can be formulated as $\sum_{k=1}^{K} r^k \beta_k$.

\textcolor{red}{\method consists of the following steps.}

\textbf{Global Prototypes Generating.}
To start with, let us rewrite the deep tabular network $F(\cdot;\theta)$ as $G_h(G_f(\cdot;\theta_f);\theta_h)$, where $G_f(\cdot;\theta_f)$ is the backbone and $G_h(\cdot;\theta_h)$ is the head parameterized by $\theta_f$ and $\theta_h$ respectively. 
To obtain global prototypes initialization, we first train $F(\cdot;\theta)$ by:
\begin{equation}
    \label{equ:org-obj}
    \min\mathcal{L}_{task}(X, Y) = \min_{\theta_f, \theta_h} \mathcal{L}(G_h\left(G_f(X; \theta_f); \theta_h\right), Y),
\end{equation}
where $\mathcal{L}$ is the loss function, and then propose applying K-Means clustering ~\citep{hartigan1979algorithm} to the output of the trained backbone $G_f(X; \theta_{f})$:
\begin{equation}
\label{K-means}
\begin{aligned}
    \min_{C\in \mathbb{R}^{K\times d}} \frac{1}{n}\sum_{i=1}^{n} \min_{\tilde{y_i}\in \{0,1\}^K} \|G_f(x_i; \theta_{f}) - \tilde{y_i}^\mathrm{T} C\|,\  \text{ subject to } \tilde{y_i}^\mathrm{T} \textbf{1}_K = 1, 
\end{aligned}
\end{equation}
where $\textbf{1}_K \in \mathbb{R}^K$ is a vector of ones, $\tilde{y_i}$ is the centroid index and $C$ is the centroid matrix.
The centroid matrix $C$ would be served as the initialization of prototypes $B$ to guide the stage (ii) training process of \method.

% The first stage involves generating task-specific prototypes for a (data, model) pair. 
% To address this, we propose applying K-Means clustering ~\citep{hartigan1979algorithm} to the output of the backbone $G_f(X; \theta_{fs})$ of trained source network:
% \begin{equation}
% \label{K-means}
% \begin{aligned}
%     \min_{C\in \mathbb{R}^{K\times d}} \frac{1}{n}\sum_{i=1}^{n} \min_{\tilde{y_i}\in \{0,1\}^K} \|G_f(x_i; \theta_{fs}) - \tilde{y_i}^\mathrm{T} C\|,\  \text{ subject to } \tilde{y_i}^\mathrm{T} \textbf{1}_K = 1, 
% \end{aligned}
% \end{equation}
% \rr{ what's the relationship between B and C?}

% Intuitively, if we initially randomize the parameters of prototypes, at the first beginning of the stage (ii) training process, both the parameters of deep tabular network $F(\cdot;\theta)$ and prototypes $B$ are random initialized, which can make it challenging for projection space to processing discriminative abilities.
% In addition, using K-Means to generate the initialization of global prototypes also enables the preservation of knowledge about the dataset structure from the trained $F(\cdot;\theta)$ in stage (i), despite the presence of noise.

The advantage of using K-Means to generate the initialization of global prototypes lies in (a) enabling the preservation of global data structure information from the trained $F(\cdot;\theta)$ in stage (i), despite the presence of noise,  and (b) facilitating a faster convergence of the stage (ii) training process compared to random initialization.


% enabling the preservation of knowledge about the dataset structure from the trained $F(\cdot;\theta)$ in stage (i), despite the presence of noise. 
% and it facilitates a faster convergence of the stage (ii) training process compared to random initialization.
% This facilitates a faster convergence of the booster model and (ii) by assigning all data points in the dataset to distinct cluster centers, K-Means captures essential global structural information present in the dataset. 

\textbf{Representation Projecting with Global Data Information via Optimal Transport.} 
After constructing the global prototypes $B$, we re-initialize the parameters of $F(\cdot;\theta)$ and start to project $F(\cdot;\theta)$'s representation into P-Space via \method to capture global data structure information.
To obtain the projection of $i$-th instance representation $G_f(x_i; \theta_f)$, we use a shared estimator $\phi(\cdot;\gamma)$ with learnable $\gamma$ to calculate its coordinate $r_i$ by $\phi(G_f(x_i; \theta_f);\gamma)$.
Mathematically, our formulation for the $i$-th projection representation distribution takes the following form: $Q_i = \sum_{k=1}^{K} r_{i}^{k} \delta_{\beta_{k}}$.
On the other hand, the $i$-th latent representation $G_f(x_i;\theta_{f})$ could be viewed as the empirical distribution over single sample representation: \hz{the notation is unclear. What's $n_j=1$?} \rr{$P_i = \delta_{G_f(x_i;\theta_{f})}$}.

Since all samples are sampled from the same data distribution, it is reasonable to assume that there exists shared structural information among these samples. 
To capture the shared global data structure information, we formulate the representation projecting as the process of extracting instance-wise data information by $G_f(x_i;\theta_{f})$ to $P_i$, and then pushing $P_i$ towards $Q_i$ to encourage each prototype $\beta_k$ to capture the shared \textit{global data structure information}, a process facilitated by leveraging the optimal transport (OT) distance:
\begin{equation}
\label{ot_loss}
\begin{aligned}
    \min\mathcal{L}_{projecting}(X, B) = \min\frac{1}{n}\sum_{i=1}^{n} \text{OT}(P_i, Q_i) = \min_{\theta_{f}, \gamma, B}  \frac{1}{n}\sum_{i=1}^{n} \langle \textbf{T}_i, \textbf{C}_i \rangle, \\
    % \text{such that }\  P_i = \sum_{j=1}^{n_j=1} \frac{1}{n_j} \delta_{x_{ij}}, Q_i = \sum_{k=1}^{K} r_{ik} \delta_{\beta_{k}}.
\end{aligned}
\end{equation}
where $\textbf{C}$ is the transport cost matrix and $\textbf{T}$ is the transport probability matrix, please refer to ~\ref{x} for more details about OT.
In contrast to the latent space of $F(\cdot;\theta)$, the P-Space consists of explicitly defined basis vectors denoted as global prototypes, thus it is more accurate to give predictions on representations within P-Space. 
We incorporate the label information by re-defining Eq.~\ref{equ:org-obj}:
\begin{equation}
\label{task specific loss}
\begin{aligned}
    \min\mathcal{L}_{task}(X, Y) = \min_{\theta_f, \theta_h, \gamma, B} \frac{1}{n}\sum_{i=1}^n \mathcal{L}(G_h(\sum_{k=1}^{K} r_i^k \beta_k;\theta_h), y_i),
\end{aligned}
\end{equation}

By representing each projected representation using the shared basis vectors (global prototypes $B$) within the P-Space, we can effectively model this \textit{global data structure information} to effectively solve one of the deep tabular network's inherent characteristic: sample localization.
The representation entanglement problem still exists within P-Space, and we will introduce the designed constraints to make the representation decoupled in the following section.


\subsection{Constraints for \method via Coordinates Diversifying and Prototype Matrix Orthogonalization} \label{sec:ptarl_constraints}
\textbf{P-Space Coordinates Diversifying Constraint}. 
Directly optimizing the above process could potentially result in a collapse of coordinates generating, which entails all projection representations exhibiting similar coordinates within P-Space. To alleviate it, we design a constraint to diversifying the coordinates towards global prototypes within P-Space to separate the representation into several disjoint regions, where representations with similar labels are in the same regions.
Specifically, for classification, we categorize samples within the same class as positive pairs ~\citep{khosla2020supervised}, while those from different classes form negative pairs. 
In the context of regression, we segment the labels within a minibatch into \(t\) sub-intervals as indicated by $t = 1 + \log(n_b)$, 
where $n_b$ is bachsize.
Samples residing within the same bin are regarded as positive pairs, while those from distinct bins are regarded as negative pairs, thereby facilitating the formation of pairings. 
This process is achieved by minimizing:
% The essence of diversifying the preference of samples for the global prototype is captured by minimizing the expression presented in Equation~\ref{diversity_loss}:
\begin{equation}
\label{diversity_loss}
\begin{aligned}
    \mathcal{L}_{diversifying}(X) = -\sum_{i=1}^{n_b}\sum_{j=1}^{n_b}\textbf{1}\{y_i, y_j \in \text{positive pair}\} \log{\frac{\exp{(\cos(r_i, r_j))}}{\sum_{i=1}^{n_b}\sum_{j=1}^{n_b} \exp{(\cos(r_i, r_j))}}}
\end{aligned}
\end{equation}
% The essence of this endeavor lies in diversifying the sample's affinity to the global prototype, a goal achieved through the minimization of Equation~\ref{diversity_loss}.

This constraint is motivated by contrastive learning (CL) ~\citep{khosla2020supervised}. 
Distinct from conventional contrastive learning methods in tabular domain that directly augment the variety of sample representations ~\citep{wang2022transtab, bahri2021scarf}, it diversifies the coordinates of latent representations within P-Space to calibrate the entangled latent representations.
% In this context, the use of prototypes as basis vectors defines a structured coordinate system in the P-Space, enhancing its clarity and making representations within it more understandable, where CL could be more effective.
In this context, the use of prototypes as basis vectors defines a structured coordinate system in the P-Space, thereby facilitating the enhancement of generating decoupled representations among samples, as opposed to directly optimizing their representations.
To improve computational efficiency, practically, we randomly select 50\% of the samples within a minibatch. 
We posit that this approach can mitigate computational complexity while makes it easier to approximate the model to the optimized state.

% \begin{equation}
% \label{diversity_loss}
% \begin{aligned}
%     \forall i, j \in minibatch, minimize(y*(-1)*(r_i \cdot r_j) + (1-y)*(r_i \cdot r_j)) \\
%     here, y=1\ if \ two \ samples'\ label\ is\ the\ same\ else\ 0
% \end{aligned}
% \end{equation}

% \subsection{Prototypes Orthogonality Regularization}
% As mentioned earlier, our goal in introducing prototype is to limit the backbone's divergence space to the implicit space of prototype, which is equivalent to the implicit space of prototype where we have to make judgments about the labels of each sample. In order to make the representation of the compressed implicit space more informative, we need each prototype to be independent of each other (if there are cases where they are not independent, this reduces the representation power of the prototype).
% In order for global prototypes to be independent of each other, we need to make them orthogonal to each other, as follows, 
\textbf{Global Prototype Matrix Orthogonalization Constraint}. 
Since the P-Space is composed of a set of global prototypes, to better represent the P-Space, these global prototypes should serve as the basis vectors, with each prototype maintaining orthogonal independence from the others. 
The presence of interdependence among prototypes would invariably compromise the representation efficacy of these prototypes.
To ensure the independence of prototypes from one another, the condition of orthogonality must be satisfied. 
This mandates the following approach:
\begin{equation}
\label{regulariz_loss}
\begin{aligned}
    % \mathcal{L}_{orthogonality}(B) = \frac{\|M\|_{1}}{\|M\|_{2}^{2}} + \max(0,|K-\|M\|_{1}|)=1, MSE(M, \mathbf{I})=0, \\
    % \mathcal{L}_{orthogonality}(B) = \frac{\|M\|_{1}}{\|M\|_{2}^{2}} + \max(0,|K-\|M\|_{1}|)=1, \\
    \min \mathcal{L}_{orthogonalization}(B) = \min (\frac{\|M\|_{1}}{\|M\|_{2}^{2}} + \max(0,|K-\|M\|_{1}|)),
    % \text{subject to }  M \in [0, 1]^{K\times K}, M_{ij} = \|\cos(\beta_i, \beta_j)\|_1,  
\end{aligned}
\end{equation}

where $M \in [0, 1]^{K\times K}$ and $M_{ij} = \|\cos(\beta_i, \beta_j)\|_1$.
The first term $\frac{\|M\|_{1}}{\|M\|_{2}^{2}}$ forces the $M$ to be sparse, i.e., any element $M_{ij} = \|\cos(\beta_i, \beta_j)\|_1$ to be close to 0 ($\beta_i$ and $\beta_j$ is orthogonal) or 1, while the second term motivates $\|M\|_{1} \to K$, i.e., only $K$ elements close to 1.
Since $M_{ii} = \|\cos(\beta_i, \beta_i)\|_1 = 1, \forall i \in K$, it would force $M_{ij} = \|\cos(\beta_i, \beta_j)\|_1, \forall i,j \in K, i \neq j$ to be 0, i.e. each prototype maintains orthogonal independence from the others.
We provide a more detailed explanation of \method and its algorithmic workflow in the Appendix ~\ref{x}.

% Altogether, the proposed method aims to minimize the following objective function w.r.t. $\theta_f, \theta_h, \theta_s$, and $B$:
% \begin{equation}
% \begin{aligned}
%     \mathcal{O}= \mathcal{L}_{task}(X, Y) + \mathcal{L}_{re-direction}(X, B) + \mathcal{L}_{diversity}(X) + \mathcal{L}_{orthogonality}(B)
%     % &\mathcal{L}( H(F(\textbf{X}; \theta_f); \theta_h), \textbf{Y})+ & \\
%     % &\mathcal{L}(OT()), \textbf{T})+ & \\
%     % &\mathcal{L}(-\sum_{i=1}^{N_b}\sum_{j=1}^{N_b}\mathbf{1}\{y_i, y_j \in positive pair\} \log{\frac{\exp{(cosine(r_i, r_j))}}{\sum_{i=1}^{N_b}\sum_{j=1}^{N_b} \exp{(cosine(r_i, r_j))}}})+ &\\
%     % &\mathcal{L}(\frac{\|M\|_{1}}{\|M\|_{2}^{2}} + \max(0,|topic\_num-\|M\|_{1}|)=1). &
% \end{aligned}
% \end{equation}

% \begin{algorithm}
% \caption{Tabular Network Booster via topic regularizing}
% \label{algorithm}
% \begin{algorithmic}[1]
% \INPUT Input data ${X, Y}$, source network $Fb$, booster network $Fn$
% \State \textbf{Initialize:} 
% \State source deep tabular model $F(\cdot;\theta_S)$
% \State train $F(\cdot;\theta_S)$ by $\argmin_{\theta_f, \theta_h}\mathcal{L}(G_h(G_f(X; \theta_f); \theta_h), Y)$
% \State obtain prototypes through adopting K-means on source backbones' hidden space $G_f(X; \theta_f)$
% \While{$B, \theta_f, \theta_h$ has not converged}
%     \State Sample minibatch $D_{\text{batch}}$ of size $B$ from $D$\;
%     \State Compute the loss OT(Pj, Qj) between Pj and Qj with Sinkhorn algorithm in Equation~\ref{ot_loss}
%     \State Random select 50\% of the samples and then compute the loss in Equation~\ref{diversity_loss}
%     \State Compute the loss in Equation~\ref{regulariz_loss} to make the global prototypes orthogonal
%     \State Compute the final loss by $\mathcal{L}(H(F(\textbf{X};\theta_f);\theta_h), \textbf{Y}) + loss_{ot} + loss_{diversity} + loss_{regularize}$
% \EndWhile
% \State update the parameters of backbone, head and global prototypes
% \end{algorithmic}
% \end{algorithm}

==> sections/rebuttal.tex <==
\section{Rebuttal}
% \textit{\textbf{We sincerely thank all reviewers for your careful reading of the manuscript and instructive advice. 
% Overall the comments are fair, encouraging, and constructive. 
% We have learned much from them. 
% The manuscript has undergone a thorough revision according to the reviewers’ comments.}
% Itemized responses to each reviewer’s comments are appended below:}

\textbf{For Reviewer 7NUi:}

We sincerely appreciate your efforts and instructive advice to improve the manuscript. We respond to each of your comments as follows:

\textbf{Q1: Unclear description of the optimization process of Eq. 4.}

R1: We are sorry for the confusion and we would like to give a more clear description. 

The Optimal Transport (OT) problem is usually to find the most cost-effective way to transform a given distribution to another distribution, which is typically achieved by calculating the specified transportation plan that minimizes the total transportation cost, while the minimized cost is usually called OT distance.
In our paper, we minimize the distance between original representation distribution over each sample $P_i$ by deep tabular models and the corresponding projection representation distribution $Q_i$ in P-Space with global prototypes, in order to preserve original data information (of $P_i$) in $Q_i$.
We follow the typical setting of OT problem to first estimate the transport plan to obtain the OT distance between $P_i$ and $Q_i$.
Then, the obtained OT distance is further used as loss function to jointly learn the two representations.

Specifically, after initializing the global prototypes $\mathcal{B}$ of P-Space, we project the original data samples into P-Space to learn the representations with global data structure information. 
To better illustrate the optimization process, we revise the Eq. 4 in the original paper to make it more readable. 
In Eq. 4, the $i$-th sample representation by deep tabular model is denoted as $G_f(x_i;\theta_f)$, the empirical distribution over this sample representation is $P_i = \delta_{G_f(x_i;\theta_f)}$, the projection representation distribution is denoted as: $Q_i = \sum_{k=1}^{K} r_{i}^{k} \delta_{\beta_{k}}$, where $r_i$ is coordinates. 
To capture the shared global data structure information, we formulate the representation projecting as the process of extracting instance-wise data information by $G_f(x_i;\theta_f)$ to $P_i$, and then pushing $P_i$ towards $Q_i$ to encourage each prototype $\beta_k$ to capture the shared global data structure information, a process achieved by minimizing the OT distance between $P_i$ and $Q_i$. 
The OT distance between $P_i$ and $Q_i$ could first be calculated by: $\text{OT}(P_i, Q_i) = \min_{\textbf{T}_i\in \Pi (P_i, Q_i)} \langle \textbf{T}_i, \textbf{C}_i \rangle$, where $C_{ik} = 1-cos(G_f(X_i;\theta_f), \beta_k)$, the average OT distance between $P_i$ and $Q_i$ over train sets could be viewed as loss function $\mathcal{L}_{projecting}(X, \mathcal{B})$ to be further optimized: $\min\mathcal{L}_{projecting}(X, \mathcal{B}) = \min\frac{1}{n}\sum_{i=1}^{n} \text{OT}(P_i, Q_i) = \min_{\theta_{f}, \gamma, \mathcal{B}}  \frac{1}{n}\sum_{i=1}^{n} \min_{\textbf{T}_i\in \Pi (P_i, Q_i)} \langle \textbf{T}_i, \textbf{C}_i \rangle$, we use gradient descent to update $\theta_f, \gamma, \mathcal{B}$. 

The idea of applying OT distances as loss functions has been employed in multiple applications. 
For example, [1] proposes using this idea for semantic segmentation, and [2] applies this idea to outlier detection in data.

[1] Importance-aware semantic segmentation in self-driving with discrete wasserstein training (Liu, Xiaofeng and Han, Yuzhuo and Bai, Song and Ge, Yi and Wang, Tianxing and Han, Xu and Li, Site and You, Jane and Lu, Jun) [AAAI 2020]

[2] Outlier-robust optimal transport (Mukherjee, Debarghya and Guha, Aritra and Solomon, Justin M and Sun, Yuekai and Yurochkin, Mikhail) [ICML 2021]


Q2: Further explanation on the \textsc{PTaRL} workflow.

R2: We have revised the workflow of \textsc{PTaRL} in Algorithm 1 in the original paper's Appendix to provide more technique details. 

As shown in the algorithm, Line 1 to 3 represents the global prototype initialization process. 
Given any deep tabular model $F(\cdot;\theta) = G_h\left(G_f(\cdot;\theta_f); \theta_h\right)$, we first train it by Eq. 2 and then apply K-Means clustering to the output of the trained backbone $G_f(\cdot;\theta_f)$ to get global prototypes $\mathcal{B}$.

From Line 4 to 19, the second stage of representation projecting is illustrated. 
The parameters of $F(\cdot;\theta)$ need to be re-initialized. 

Line 8 to 14 details the process of calculating $\mathcal{L}_{projecting}$.
Within a minibatch, for each instance, we calculate the OT distance between its representation by the deep tabular model and the projection representation in P-Space.
We then average the OT distance of each instance within the minibatch as the $\mathcal{L}_{projecting}$.
In Line 12, $C_i$ is the transport cost matrix calculated by cosine distance: $C_{ik} = 1-cos(G_f(X_i;\theta_f), \beta_k)$.
The $\mathcal{L}_{projecting}$ would be further optimized to push $P_i$ towards $Q_i$ to encourage each prototype to capture the shared global data structure information.

We introduce $\mathcal{L}_{task}$ in Line 15 to incorporate task-specific label supervision.
$\mathcal{L}_{diversifying}$ in Line 16 is introduced as the P-Space Coordinates Diversifying Constraint to alleviate the collapse of coordinates generating.
Additionally, $\mathcal{L}_{orthogonalization}$ in Line 17 serves as the Global Prototype Matrix Orthogonalization Constraint, ensuring the independence of global prototypes from each other.
Here, $M \in [0, 1]^{K\times K}$ and $M_{ij} = \|\cos(\beta_i, \beta_j)\|_1$. 


Q3: Unclear description in the illustration of Fig. 2.

R3: Thanks very much for pointing this confusion. We have revised our Fig. 2 in the original paper. 

We have clarified the hidden representation in Phase 1 and the projection representation in Phase 2. 
In phase 1, given any deep tabular model $F(\cdot;\theta) = G_h\left(G_f(\cdot;\theta_f); \theta_h\right)$, 
we initially train it with Eq. 2. Subsequently, K-Means clustering is applied to the output of the trained backbone $G_f(\cdot;\theta_f)$ to obtain global prototypes $\mathcal{B}$ for constructing P-Space.
Moving on to Phase 2, $G_f(\cdot;\theta_f)$ and $G_h(\cdot;\theta_h)$ are re-initialized as $G_f(\cdot;\theta_f^*)$ and $G_h(\cdot;\theta_h^*)$.
The representation generated by $G_f(\cdot;\theta_f^*)$ is then projected into P-Space to learn the projection representation, denoted as ``Space Calibration'' in Fig. 2.
In this process, a shared coordinates estimator calculates coordinates for the projection in P-Space, and then the projection representation is obtained by $\sum_{k=1}^{K} r_{i}^{k} {\beta_{k}}$. 
The projection representation in P-Space would be finally processed by $G_h(\cdot;\theta_h^*)$ to give predictions.  

Moreover, we give further explanation about the three sentences on the right side of Fig. 2.
``Projecting Via Optimal Transport'' indicates that the representation by $G_f(\cdot;\theta_f^*)$ is pushed forward to projection representation by minimizing the Optimal Transport Distance between the two representations.
The sentences ``coordinates diversifying'' and ``prototypes orthogonalization'' correspond to two constraints for representation disentanglement, i.e. P-Space Coordinates Diversifying Constraint and Global Prototype Matrix Orthogonalization Constraint.



\textbf{For Reviewer z5Xh:}
We sincerely appreciate your efforts and instructive advice to improve the manuscript. We respond to each of your comments as follows:

W1: Further experimental results of applying \textsc{PTaRL} to recent deep models for tabular representation.

R1: Thanks for your valuable suggestion. We have applied \textsc{PTaRL} to recent deep tabular model SAINT, making it one of our baseline models.
We provide additional experiment results in Section 6 Table 1, Appendix Table 5 and Table 6.
The main results as follows:  

\begin{table}[h]
\centering
\setlength{\tabcolsep}{2.5mm}{
\begin{tabular}{c|cccccc|c}
\toprule
                                           & AD $\uparrow$  & HI $\uparrow$  & HE $\uparrow$  & JA $\uparrow$  & AL $\uparrow$  & CA $\downarrow$     & Win         \\ \midrule
SAINT                                      & 0.826          & 0.689          & 0.363          & 0.675          & 0.913          & 0.492               & 0           \\ \hline  
SAINT + \textsc{PTaRL}                     & \textbf{0.861} & \textbf{0.728} & \textbf{0.401} & \textbf{0.728} & \textbf{0.950} & \textbf{0.471}      & 6           \\
\bottomrule
\end{tabular}}
\end{table}

The results show that \textsc{PTaRL} has the ability to generally improve deep tabular models' performance, including recently proposed models such as SAINT. 


Q1: Can the proposed \textsc{PTaRL} be applied to generative models?

R2: 
Thanks for your constructive suggestion.
We hope that our proposed method could offer valuable insights to enhance generative model representations and it will be an important direction for our future work.
Take the research line of deep generative models for representation learning as an example.
Deep generative models excel in discerning the true data distribution by learning the distribution of input data within the latent space. 
In this context, the representation of data in the latent space serves as a comprehensive data representation. 
It appears that \textsc{PTaRL} offers a potential solution to incorporate global data information through prototypes.
Leveraging such global data information to enhance the representation of latent structures aids in better modeling the true data distribution, consequently improving the generative model's performance. 


\textbf{For Reviewer Gxco:} 
Thanks for your comments. We respond to your questions as follows and hope they can address your concerns.


Q1: Unclear definition of the concepts of \textit{global data structure information} and \textit{sample localization}.

R1: 
%We apologize for any confusion and appreciate the opportunity to provide a more explicit description of both ``global data structure information'' and ``sample localization''.
In the context of any tabular dataset, we have observed \textit{global data structure information} comprises two different components: (i) the global feature structure and (ii) the global sample structure.

Considering the feature structure, traditional and deep tabular machine learning methods utilize all features or a subset of features as input, allowing them to model inherent interactions among features and thereby acquire a comprehensive global feature structure.
In addition, there also exists the sample structure given a tabular dataset. Traditional methods (e.g., boosted trees) can effectively model the overarching relationships between data samples. Specifically, in XGBoost, the dataset undergoes partitioning by comparing all the samples, with each node of a decision tree representing a specific partition, and each leaf node corresponding to a predictive value. The iterative splitting of nodes during training empowers decision trees in XGBoost to learn the distribution of all the samples across distinct regions of the data space, capturing global sample structure.


However, we note that deep tabular machine learning methods typically rely on batch training to obtain data representations within a batch. These methods do not explicitly consider the structure between samples within a batch. %The learned localized structure of a batch encapsulates the essence of "sample localization" as discussed in our paper.
Furthermore, they fail to capture the global structure between samples across different batches. This limitation presents challenges in comprehensively capturing global data distribution information, consequently impeding overall performance.

Our methods rebuild the representation space with global prototypes (P-Space) in the first stage.
Then in the second stage, the original data representation by deep tabular machine learning methods is projected into P-Space to obtain projection representation with global prototypes. 
On the one hand, by minimizing the Optimal Transport distance between the two representations, we could represent each sample with global prototypes, and in the meanwhile encode the global feature structure in learning global prototypes, considering backbone models can inherently learn the interactions among features.
On the other hand, the global prototypes are learned by directly modeling all the data samples and thus the complex data distribution could be obtained by global prototypes to capture the global sample structure.  
% all samples are sampled from the same data distribution, by explicitly modeling each sample with global prototypes, the complex data distribution could be obtained by global prototypes to capture (2) global sample structure.  
Therefore, \textsc{PTaRL} is able to capture both the feature and sample structure information by prototype learning. Considering previous deep tabular machine learning methods can only acquire the representations limited by the batch training, we use the concept of \textit{sample localization} to encapsulate this limitation.
% %The learned localized structure of a batch encapsulates the essence of "sample localization" as discussed in our paper.

Q2: Doubts about the Fig. 1 and Fig. 4. 

R2: 
Thanks for your mention. 
We also note that there exists certain overlap in Fig. 1. 
% After our careful analysis, we the difference between Fig. 1 and Fig. 4 is resulted from the different characteristics of distinct datasets ([SUMMARIZE])
After our careful analysis, we attribute the differences between Fig. 1 and Fig. 4 to the different characteristics of distinct datasets. 

Specifically, Fig. 1 is based on the Adult dataset, while Fig. 4 is derived from the Higgs and Jannis datasets.
In comparison to the Higgs dataset (98050 samples, 28 features) and the Jannis dataset (83733 samples, 54 features), the Adult dataset (48842 samples, 14 features) has a smaller number of samples and features. 
Additionally, the Adult dataset includes both numerical and categorical features, whereas the Higgs and Jannis datasets only contain numerical features. 
Considering the smaller size of the Adult dataset for training and its more intricate feature relationships, it poses a more challenging task for deep tabular machine learning methods to learn disentangled representations.
Our proposed \textsc{PTaRL} offers a viable solution to enhance the disentanglement of representations by deep tabular machine learning methods.

% Challenging --> Model hard to learn/distinguish/classify/ overlap,
% howoever, with our PTARL, our enhance distinguishment 


Q3: Unclear description of the diversification in Fig. 5.  

R3: We apologize for any confusion and have enhanced the clarity of Fig. 5 for improved illustration.
The top and bottom rows respectively depict scenarios without and with the Diversifying Constraint.
The first and second columns represent the mean coordinate values of two distinct categories, while the third column illustrates the difference between the two categories.
The first row shows that without Diversifying Constraint, the average coordinates between two different categories are similar, posing challenges in effectively distinguishing representations belonging to distinct categories.
Contrastingly, the second row, which introduces the Diversifying Constraint, showcases a more pronounced difference in coordinates between categories, thereby promoting diversification in the coordinates of distinct categories.

Q4.1: Comparison between \textsc{PTaRL} and state-of-the-art tree-based methods. 

R4.1: Thanks for valuable suggestion. We have conducted a comparison of the performance of \textsc{PTaRL} (utilizing FT-Transformer as a backbone) with two state-of-the-art tree-based methods, namely XGBoost and LightGBM.
The experimental results are detailed below and can also be referenced in Table 9 in the Appendix.
In comparison to XGBoost, \textsc{PTaRL} performs better across all experimental settings.
When contrasted with LightGBM, \textsc{PTaRL} outperforms it in 4 out of 6 settings, with a slight performance dip observed in the remaining 2 settings.
In summary, \textsc{PTaRL} consistently matches the performance of state-of-the-art tree-based methods across various settings. 
The utilization of deep learning for tabular data, allowing the construction of multi-model pipelines and knowledge transfer across different domains, is an appealing prospect. Our proposed method holds the potential to enhance the application of deep learning in the tabular domain.



\begin{table}
\centering
\setlength{\tabcolsep}{2.5mm}{
\begin{tabular}{c|cccccc}
\toprule
                                                 & AD $\uparrow$  & HI $\uparrow$  & HE $\uparrow$  & JA $\uparrow$  & AL $\uparrow$  & CA $\downarrow$        \\ \midrule
XGBoost                                          & 0.856          & 0.691          & 0.361          & 0.724          & 0.954          & 0.462         \\
LightGBM                                         & 0.860          & 0.713          & 0.382          & \textbf{0.743} & 0.968          & \textbf{0.445}\\
FT-Transformer + \textsc{PTaRL}                  & \textbf{0.871} & \textbf{0.738} & \textbf{0.397} & 0.738          & \textbf{0.97}  & 0.448         \\
\bottomrule
\end{tabular}}
\end{table}

Q4.2: Comparison between \textsc{PTaRL} and other classical machine learning methods.

R4.2: Thanks for constructive suggestion. We compare the performance of \textsc{PTaRL} (with FT-Transformer as backbone) and two classical machine learning methods 
, namely Support Vector Machine (SVM) for classification, Support Vector Regression (SVR) for regression, and K-Nearest Neighbors (KNN). 
The detailed experimental results are provided below and can also be referenced in Table 10 in the Appendix.
The results show that \textsc{PTaRL} performs significantly better than SVM, SVR, and KNN. 
% The results demonstrate that using our method plays a big role for table deep learning

\begin{table}
\centering
\setlength{\tabcolsep}{2.5mm}{
\begin{tabular}{c|cccccc}
\toprule
                                                 & AD $\uparrow$  & HI $\uparrow$  & HE $\uparrow$  & JA $\uparrow$  & AL $\uparrow$  & CA $\downarrow$        \\ \midrule
SVM (SVR for regression)                         & 0.823          & 0.683          & 0.340          & 0.658          & 0.901          & 0.515                  \\ 
KNN                                              & 0.816          & 0.680          & 0.345          & 0.652          & 0.889          & 0.522                  \\
FT-Transformer + \textsc{PTaRL}                  & \textbf{0.871} & \textbf{0.738} & \textbf{0.397} & \textbf{0.738} & \textbf{0.97}  & \textbf{0.448}         \\
\bottomrule
\end{tabular}}
\end{table}

Q4.3: The influence of DNN depths to the performance of \textsc{PTaRL}. 

R4.3: 
Thank you for the insightful suggestion. We employed MLP and FT-Transformer as our two backbone models to examine the impact of DNN depths on the performance of \textsc{PTaRL}.
The experiments involved gradually increasing the depths of these backbones, and subsequently evaluating the model performance across three datasets encompassing binary classification, multiclass classification, and regression tasks. 
The detailed experimental results are presented below and can also be found in Table 11 in the Appendix.
The outcomes indicate that, in the absence of \textsc{PTaRL}, augmenting the model depth does not consistently enhance performance; in fact, there is a decline in performance when the depth becomes excessively deep. Contrastingly, when applying \textsc{PTaRL}, the model exhibits remarkable robustness across varying depths. We posit that the utilization of global prototypes for representations in P-Space, as incorporated in the proposed \textsc{PTaRL}, significantly contributes to this observed effect.

\begin{table}
\centering
\setlength{\tabcolsep}{2.5mm}{
\begin{tabular}{c|c|cccccc}
\toprule
Datasets & Models                                  & layers = 3     & layers = 5     & layers = 7     & layers = 9     \\ \midrule 
\multirow{4}{*}{HI $\uparrow$ }      & MLP         & 0.680          & 0.707          & 0.675          & 0.669          \\
& MLP + \textsc{PTaRL}                             & \textbf{0.719} & \textbf{0.730} & \textbf{0.729} & \textbf{0.732} \\
& FT-Transformer                                   & 0.687          & 0.719          & 0.709          & 0.691          \\
& FT-Transformer + \textsc{PTaRL}                  & \textbf{0.738} & \textbf{0.742} & \textbf{0.741} & \textbf{0.737} \\
\bottomrule
\toprule
\multirow{4}{*}{JA $\uparrow$ }      & MLP         & 0.670          & 0.715          & 0.704          & 0.689          \\
& MLP + \textsc{PTaRL}                             & \textbf{0.708} & \textbf{0.732} & \textbf{0.728} & \textbf{0.733} \\
& FT-Transformer                                   & 0.689          & 0.716          & 0.729          & 0.709          \\
& FT-Transformer + \textsc{PTaRL}                  & \textbf{0.738} & \textbf{0.741} & \textbf{0.745} & \textbf{0.742} \\
\bottomrule
\toprule
\multirow{4}{*}{CA $\downarrow$ }    & MLP         & 0.522          & 0.513          & 0.509          & 0.524          \\ 
& MLP + \textsc{PTaRL}                             & \textbf{0.491} & \textbf{0.480} & \textbf{0.482} & \textbf{0.479} \\
& FT-Transformer                                   & 0.486          & 0.476          & 0.472          & 0.478          \\
& FT-Transformer + \textsc{PTaRL}                  & \textbf{0.448} & \textbf{0.446} & \textbf{0.442} & \textbf{0.443} \\
\bottomrule
\end{tabular}}
\end{table}

% Summary:
We would like to express our sincere gratitude for your insightful suggestions which have significantly contributed to the refinement of our paper. Classical methodologies, such as XGBoost, KNN, and SVM, enjoy widespread adoption among practitioners for solving tabular problems, owing to their commendable performance and user-friendly nature. The comparative analysis between deep learning models and traditional approaches is instrumental in advancing the overall model generality within the tabular domain. We hope that our proposed method could offer valuable insights to the community. 

%the enhancement of traditional methodologies.

==> sections/rebuttal_original.tex <==
\section{Rebuttal}
% \textit{\textbf{We sincerely thank all reviewers for your careful reading of the manuscript and instructive advice. 
% Overall the comments are fair, encouraging, and constructive. 
% We have learned much from them. 
% The manuscript has undergone a thorough revision according to the reviewers’ comments.}
% Itemized responses to each reviewer’s comments are appended below:}

\textbf{For Reviewer 7NUi:}

We sincerely appreciate your efforts and instructive advice to improve the manuscript! We respond to each of your comments as follows:

\textbf{Q1: Unclear description of the optimization process of Eq.4.}

R1: We are sorry for the confusion and we would like to give a more clear description. 

The Optimal Transport (OT) problem is usually to find the most cost-effective way to transform a given distribution to another distribution (OT distance), it is typically achieved by calculating the specified transportation plan that minimizes the total transportation cost. 
In our paper, we minimize the distance between original instance representation distribution $P_i$ by deep tabular models and the projection representation distribution $Q_i$ in P-Space with global prototypes, to push $P_i$ towards $Q_i$ to preserve original data structure information.
We follow the typical setting of OT problem to first estimate the transport plan to obtain the OT distance between $P_i$ and $Q_i$.
In addition, the obtained OT distance is further used as loss function to be optimized to jointly optimize the original representations by deep tabular models and projection representations in P-Space.

Specifically, after initializing the global prototypes $\mathcal{B}$ in P-Space, we project the original data samples into P-Space to learn the representations with global data structure information. 
To better illustrate the optimization process, we revise the Eq.4 in original paper to make it more readable. In Eq.4, the $i$-th sample representation by backbone is denoted as $G_f(x_i;\theta_f)$, the empirical distribution over this sample representation is $P_i = \delta_{G_f(x_i;\theta_f)}$, the projection representation distribution is denoted as: $Q_i = \sum_{k=1}^{K} r_{i}^{k} \delta_{\beta_{k}}$, where $r_i$ is coordinates. To capture the shared global data structure information, we formulate the representation projecting as the process of extracting instance-wise data information by $G_f(x_i;\theta_f)$ to $P_i$, and then pushing $P_i$ towards $Q_i$ to encourage each prototype $\beta_k$ to capture the shared global data structure information, a process achieved by minimizing the OT distance between $P_i$ and $Q_i$. The OT distance between $P_i$ and $Q_i$ could first be calculated by: $\text{OT}(P_i, Q_i) = \min_{\textbf{T}_i\in \Pi (P_i, Q_i)} \langle \textbf{T}_i, \textbf{C}_i \rangle$, where $C_{ik} = 1-cos(G_f(X_i;\theta_f), \beta_k)$, the average OT distance between $P_i$ and $Q_i$ over train sets could be viewed as loss function to be further optimized: $\min \mathcal{L}_{projecting}(X, \mathcal{B}) = \min\frac{1}{n}\sum_{i=1}^{n} \text{OT}(P_i, Q_i) = \min_{\theta_{f}, \gamma, \mathcal{B}}  \frac{1}{n}\sum_{i=1}^{n} \min_{\textbf{T}_i\in \Pi (P_i, Q_i)} \langle \textbf{T}_i, \textbf{C}_i \rangle$, we use gradient descent to update $\theta_f, \gamma, \mathcal{B}$.

Q2: Further explanation on the \textsc{PTaRL} workflow.

R to Q2: We are sorry for the confusion and we have revised the workflow of \textsc{PTaRL} in original paper Appendix Algorithm 1 to provide more technique details. 
We also provide the detailed algorithm as follows:

\begin{algorithm}
% \caption{\textsc{PTaRL} algorithm workflow.}
% \label{algorithm}
\begin{algorithmic}[1]
\INPUT Input data $D=\{X, Y\}$, deep tabular model $F(\cdot;\theta) = G_h\left(G_f(\cdot;\theta_f); \theta_h\right)$, coordinates estimator $\phi(\cdot;\gamma)$
% \State \textbf{Initialize:} 
\State \textbf{Phase 1: prototype generating} 
\State Train $F(\cdot;\theta)$ by $\min\mathcal{L}_{task}(X, Y) = \min_{\theta_f, \theta_h} \mathcal{L}(G_h\left(G_f(X; \theta_f); \theta_h\right), Y)$ (Eq.2)
\State Obtain global prototypes $\mathcal{B} = \{\beta_k\}_{k=1}^K \in \mathbb{R}^{K\times d}$ through applying K-Means clustering to the output of the trained backbone $G_f(X; \theta_{f})$
\State \textbf{Phase 2: representation projecting} 
\State Re-initialize the parameters of $F(\cdot;\theta) = G_h\left(G_f(\cdot;\theta_f); \theta_h\right)$
\While{$\mathcal{B}, \theta_f, \theta_h, \gamma$ has not converged}
    \State Sample minibatch of size $n_b$ from $D$\;
    \For{$i \gets 1$ to $n_b$}
        \State Obtain $i$-th instance representation distribution by $P_i = \delta_{G_f(x_i;\theta_{f})}$ 
        \State Calculate $i$-th instance projection representation coordinates $r_i = \phi(G_f(x_i; \theta_f);\gamma)$
        \State Obtain $i$-th instance projection representation distribution: $Q_i = \sum_{k=1}^{K} r_{i}^{k} \delta_{\beta_{k}}$
        \State Calculate the OT distance between $P_i$ and $Q_i$: $\text{OT}(P_i, Q_i) = \min_{\textbf{T}_i\in \Pi (P_i, Q_i)} \langle \textbf{T}_i, \textbf{C}_i \rangle$
        % \State Projecting instance representation into P-Space by Eq.~\ref{ot_loss}
    \EndFor
    \State Average the OT distance within the minibatch to compute $\mathcal{L}_{projecting}(X, \mathcal{B}) = \frac{1}{n_b}\sum_{i=1}^{n_b} \text{OT}(P_i, Q_i) = \frac{1}{n_b}\sum_{i=1}^{n_b} \min_{\textbf{T}_i\in \Pi (P_i, Q_i)} \langle \textbf{T}_i, \textbf{C}_i \rangle$ (Eq.4)
    \State Compute $\mathcal{L}_{task}(X, Y) = \frac{1}{n_b}\sum_{i=1}^{n_b} \mathcal{L}(G_h(\sum_{k=1}^{K} r_i^k \beta_k;\theta_h), y_i)$ (Eq.5)
    \State Random select 50\% of the samples within minibatch to compute $\mathcal{L}_{diversifying}(X) = -\sum_{i=1}^{n_b}\sum_{j=1}^{n_b}\textbf{1}\{y_i, y_j \in \text{positive pair}\} \log{\frac{\exp{(\cos(r_i, r_j))}}{\sum_{i=1}^{n_b}\sum_{j=1}^{n_b} \exp{(\cos(r_i, r_j))}}}$ (Eq.6)
    \State Compute $\mathcal{L}_{orthogonalization}(\mathcal{B}) = (\frac{\|M\|_{1}}{\|M\|_{2}^{2}} + \max(0,|K-\|M\|_{1}|))$ (Eq.7)
    \State Update $\theta_f, \theta_h, \gamma, \mathcal{B}$ by optimizing $\mathcal{L}_{projecting}, \mathcal{L}_{task}, \mathcal{L}_{diversifying}, \mathcal{L}_{orthogonalization}$
\EndWhile
\State \Return $G_f, G_h, \phi, \mathcal{B}$
\end{algorithmic}
\end{algorithm}

As shown in the algorithm, line 1 to 3 represents the global prototype initialization process, given any deep tabular model $F(\cdot;\theta) = G_h\left(G_f(\cdot;\theta_f); \theta_h\right)$, we first train it by Eq.2 and then apply K-Means clustering to the output of the trained backbone $G_f(\cdot;\theta_f)$ to get global prototypes $\mathcal{B}$.
The second stage of representation projecting is start from the line 4. 
The parameters of $F(\cdot;\theta)$ should be re-initialized.
Then within a minibatch, for each instance, we calculate the OT distance between its representation by deep tabular model and projection representation in P-Space.
We average the OT distance of each instance within the minibatch as the $\mathcal{L}_{projecting}$ (Line 8 to 14).
In line 12, $C_i$ is the transport cost matrix calculated by cosine distance: $C_{ik} = 1-cos(G_f(X_i;\theta_f), \beta_k)$.
The $\mathcal{L}_{projecting}$ would be further optimized to push $P_i$ towards $Q_i$ to encourage each prototype to capture the shared global data structure information.
We add $\mathcal{L}_{task}$ in line 15 to provide task-specific label supervision.
We add $\mathcal{L}_{diversifying}$ in line 16 as the P-Space Coordinates Diversifying Constraint to alleviate the collapse of coordinates generating.
We also add $\mathcal{L}_{orthogonalization}$ in line 17 as Global Prototype Matrix Orthogonalization Constraint to ensure the independence of global prototypes from one another. 
Here, $M \in [0, 1]^{K\times K}$ and $M_{ij} = \|\cos(\beta_i, \beta_j)\|_1$.


Q3: Unclear description in the illustration of Fig. 2.

R to Q3: 
We are sorry for the confusion and we have revised the Fig.2 in original paper.
We would like to give a more clear description to illustrate Fig.2 as follows.
The left and right part correspond to phase 1: prototype generating and phase 2: representation projecting respectively.
Phase 2 would start after phase 1 is finished.
In phase 1, given any deep tabular model $F(\cdot;\theta) = G_h\left(G_f(\cdot;\theta_f); \theta_h\right)$, we first train it by Eq.2 and then apply K-Means clustering to the output of the trained backbone $G_f(\cdot;\theta_f)$ to get global prototypes $\mathcal{B}$ to construct P-Space.
In phase 2, $G_f(\cdot;\theta_f), G_h(\cdot;\theta_h)$ would first be re-initialized to be $G_f(\cdot;\theta_f^*), G_h(\cdot;\theta_h^*)$.
The representation generated by $G_f(\cdot;\theta_f^*)$ should be projected into P-Space to learn projection representation, which is labeled as Space Calibration in Fig.2.
In Space Calibration, we use a shared coordinates estimator to calculate coordinates for projection in P-Space. 
Then the projection representation is obtained by $\sum_{k=1}^{K} r_{i}^{k} {\beta_{k}}$.
The representation by $G_f(\cdot;\theta_f^*)$ is pushing forward to projection representation via minimizing the Optimal Transport Distance between the two representations.
The two sentences ``coordinates diversifying'' and ``prototypes orthogonalization'' correspond to two constraints for representation disentangled, i.e. P-Space Coordinates Diversifying Constraint and Global Prototype Matrix Orthogonalization Constraint.
The projection representation in P-Space would be finally processed by $G_h(\cdot;\theta_h^*)$ to give predictions.

\textbf{For Reviewer z5Xh:}
We sincerely appreciate your efforts and instructive advice to improve the manuscript! We respond to each of your comments one-by-one in the following (W represents weakness, Q represents question and R represents response).

W1: Further experimental results of applying PTaRL to recent deep models for tabular representation.

R to W1: Thanks for your valuable suggestion! We have applied \textsc{PTaRL} to recent deep tabular model: SAINT, and we have involved SAINT as one of our baseline models. 
We provide additional experiment results in Section 6 Table 1, Appendix Table 5 and Table 6.
The main results as follows:  

\begin{table}[h]
\centering
\setlength{\tabcolsep}{2.5mm}{
\begin{tabular}{c|cccccc|c}
\toprule
                                           & AD $\uparrow$  & HI $\uparrow$  & HE $\uparrow$  & JA $\uparrow$  & AL $\uparrow$  & CA $\downarrow$     & Win         \\ \midrule
SAINT                                      & 0.826          & 0.689          & 0.363          & 0.675          & 0.913          & 0.492               & 0           \\ \hline  
SAINT + \textsc{PTaRL}                     & \textbf{0.861} & \textbf{0.728} & \textbf{0.401} & \textbf{0.728} & \textbf{0.950} & \textbf{0.471}      & 6           \\
\bottomrule
\end{tabular}}
\end{table}

The results show that \textsc{PTaRL} has the ability to generally improve deep tabular models' performance, including recently proposed models such as SAINT.

Q1: Can the proposed PTaRL be applied to generative models?

R to Q1: 
Thanks for your great suggestion!
We believe that our core idea could be applied to enhance generative model representations and it will be an important direction for our future work.
Take the research line of deep generative models for representation learning as example.
Deep generative models excel in discerning the true data distribution by learning the distribution of input data within the latent space. 
In this context, the representation of data in the latent space serves as a comprehensive data representation. 
However, during batch training, the absence of explicitly considering the global data structure between samples within the total train set may drop into sample localization. 
One viable solution lies in the application of our proposed prototype learning method to delineate the latent representations. 
By employing a set of global prototypes that encapsulates global data structure information, each latent representation can be effectively characterized. 
Leveraging global data information to enhance the representation of latent structures aids in better modeling the true data distribution, consequently improving the generative model's performance.


\textbf{For Reviewer Gxco:} 
We sincerely appreciate your efforts and instructive advice to improve the manuscript! We respond to each of your comments one-by-one in the following (W represents weakness, Q represents question and R represents response).

Q1: Unclear definition of the concepts of “global data structure information” and “sample localization”.

R to Q1: 
We apologize for any confusion and appreciate the opportunity to provide a more explicit description of both "global data structure information" and "sample localization."

In the context of a complete tabular dataset, “global data structure information” comprises two fundamental components: (1) the global feature structure and (2) the global sample structure.

Considering the global feature structure, traditional and deep tabular machine learning methods utilize all or a subset of features as input, allowing them to model inherent interactions among features and thereby acquire a comprehensive global feature structure.

For the global sample structure, decision tree-based methods, such as XGBoost, can effectively model the overarching relationships between samples. In XGBoost, the dataset undergoes partitioning by comparing samples, with each node of a decision tree representing a specific partition, and each leaf node corresponding to a predictive value. The iterative splitting of nodes during training empowers decision trees in XGBoost to learn the distribution of samples across distinct regions of the feature space, capturing intricate relationships among samples.

It is essential to note that deep machine learning tabular methods typically rely on batch training to obtain instance representations within a batch. These methods, however, do not explicitly consider the structure between samples within a batch, encapsulating the essence of "sample localization" as discussed in our paper.

Furthermore, deep machine learning tabular methods fail to capture the "global" structure between samples across different batches. This limitation presents challenges in comprehensively capturing global data distribution information, consequently impeding overall performance.

Our methods rebuild the representation space with global prototypes (P-Space) in the first stage.
Then in the second stage, each instance representation by backbone is projected into P-Space to obtain projection representation with global prototypes. 
By minimizing the Optimal Transport distance between the two representations, we could represent each sample with global prototypes. 
Since backbone models could model the inherent interactions among features, by pushing instance representation of backbone towards projection representation in P-Space, the (1) global feature structure is transformed into global prototypes.
In addition, all samples are sampled from the same data distribution, by explicitly modeling each sample with global prototypes, the complex data distribution could be obtained by global prototypes to capture (2) global sample structure.  
Therefore, \textsc{PTaRL} is able to capture the global data structure information by prototype learning.

Q2: Doubts about the Figure 1 and Figure 4. 

R to Q2: We are sorry for the visualization results that there still exists substantial overlap in Figure 1.
Figure 1 is conducted on Adult dataset, while Figure 4 is conducted on Higgs and Jannis datasets.
Compared to Higgs (98050 samples, 28 features) and Jannis (83733 samples, 54 features) datasets, Adult (48842 samples, 14 features) dataset has smaller samples and feature numbers. 
In addition, Adult consists of both numerical and categorical features, while Higgs and Jannis only have numercial features.
Compared to Higgs and Jannis, Adult has smaller data samples for training and more complex feature relationships, thus it is a more challenge task to achieve representation disentanglement on Adult.

Q3: Unclear description of the diversification in Fig. 5.  

R to Q3: We apologize for any confusion and have enhanced the clarity of Fig. 5 for improved illustration.
The top and bottom rows respectively depict scenarios without and with the Diversifying Constraint.
The first and second columns represent the mean coordinate values of two distinct categories, while the third column illustrates the difference between the two categories.
The first row shows that without Diversifying Constraint, the average coordinates between two different categories are similar, posing challenges in effectively distinguishing representations belonging to distinct categories.
Contrastingly, the second row, which introduces the Diversifying Constraint, showcases a more pronounced difference in coordinates between categories, thereby promoting diversification in the coordinates of distinct categories.

Q4.1: Comparison between \textsc{PTaRL} and state-of-the-art tree-based methods. 

R to Q4.1: Thanks for valuable suggestion! We compare the performance of \textsc{PTaRL} (with FT-Transformer as backbone) and two state-of-the-art tree-based methods XGBoost, LightGBM as follows. 
In comparison to XGBoost, \textsc{PTaRL} performs better across all experimental settings.
When contrasted with LightGBM, \textsc{PTaRL} outperforms it in 4 out of 6 settings. However, in the settings JA and CA where \textsc{PTaRL} exhibits a slight performance dip.
In summary, \textsc{PTaRL} consistently matches the performance of state-of-the-art tree-based methods across various settings. 
The utilization of deep learning for tabular data, allowing the construction of multi-model pipelines and knowledge transfer across different domains, is an appealing prospect. Our proposed method holds the potential to enhance the application of deep learning in the tabular domain.


\begin{table}
\centering
\setlength{\tabcolsep}{2.5mm}{
\begin{tabular}{c|cccccc}
\toprule
                                                 & AD $\uparrow$  & HI $\uparrow$  & HE $\uparrow$  & JA $\uparrow$  & AL $\uparrow$  & CA $\downarrow$        \\ \midrule
XGBoost                                          & 0.856          & 0.691          & 0.361          & 0.724          & 0.954          & 0.462         \\
LightGBM                                         & 0.860          & 0.713          & 0.382          & \textbf{0.743} & 0.968          & \textbf{0.445}\\
FT-Transformer + \textsc{PTaRL}                  & \textbf{0.871} & \textbf{0.738} & \textbf{0.397} & 0.738          & \textbf{0.97}  & 0.448         \\
\bottomrule
\end{tabular}}
\end{table}

Q4.2: Comparison between \textsc{PTaRL} and older ML methods, such as prototype and kernel based methods.

R to Q4.2: Thanks for great suggestion! We compare the performance of \textsc{PTaRL} (with FT-Transformer as backbone) and two classical prototype and kernel methods SVM for classification (SVR for regression), KNN as follows.
The results show that \textsc{PTaRL} performs significantly better than KNN, SVM and SVR.

\begin{table}
\centering
\setlength{\tabcolsep}{2.5mm}{
\begin{tabular}{c|cccccc}
\toprule
                                                 & AD $\uparrow$  & HI $\uparrow$  & HE $\uparrow$  & JA $\uparrow$  & AL $\uparrow$  & CA $\downarrow$        \\ \midrule
KNN                                              & 0.816          & 0.680          & 0.345          & 0.652          & 0.889          & 0.522                  \\
SVM (SVR for regression)                         & 0.823          & 0.683          & 0.340          & 0.658          & 0.901          & 0.515                  \\ 
FT-Transformer + \textsc{PTaRL}                  & \textbf{0.871} & \textbf{0.738} & \textbf{0.397} & \textbf{0.738} & \textbf{0.97}  & \textbf{0.448}         \\
\bottomrule
\end{tabular}}
\end{table}

Q4.3: The influence of DNN depths to the performance of \textsc{PTaRL}. 

R to Q4.3: 
Thank you for the insightful suggestion! We employed MLP and FT-Transformer as our two backbone models. The approach involved gradually increasing the depths of these backbones, and subsequently evaluating the model performance across three datasets encompassing binary classification, multiclass classification, and regression tasks.
The outcomes indicate that, in the absence of \textsc{PTaRL}, augmenting the model depth does not consistently enhance performance; in fact, there is a decline in performance when the depth becomes excessively deep. Contrastingly, when applying \textsc{PTaRL}, the model exhibits remarkable robustness across varying depths. We posit that the utilization of global prototypes for representations in P-Space, as incorporated in the proposed \textsc{PTaRL}, significantly contributes to this observed effect.

\begin{table}
\centering
\setlength{\tabcolsep}{2.5mm}{
\begin{tabular}{c|c|cccccc}
\toprule
Datasets & Models                                  & layers = 3     & layers = 5     & layers = 7     & layers = 9    \\ \midrule 
\multirow{4}{*}{HI $\uparrow$ }      & MLP         & 0.680          & 0.707          & 0.675          & 0.669         \\
& MLP + \textsc{PTaRL}                             & 0.719          & 0.730          & 0.729          & 0.732         \\
& FT-Transformer                                   & 0.687          & 0.719          & 0.709          & 0.691         \\
& FT-Transformer + \textsc{PTaRL}                  & 0.738          & 0.742          & 0.741          & 0.737         \\
\bottomrule
\toprule
\multirow{4}{*}{JA $\uparrow$ }      & MLP         & 0.670          & 0.715          & 0.704          & 0.689         \\
& MLP + \textsc{PTaRL}                             & 0.708          & 0.732          & 0.728          & 0.733         \\
& FT-Transformer                                   & 0.689          & 0.716          & 0.729          & 0.709         \\
& FT-Transformer + \textsc{PTaRL}                  & 0.738          & 0.741          & 0.745          & 0.742         \\
\bottomrule
\toprule
\multirow{4}{*}{CA $\downarrow$ }    & MLP         & 0.522          & 0.513          & 0.509          & 0.524         \\ 
& MLP + \textsc{PTaRL}                             & 0.491          & 0.480          & 0.482          & 0.479         \\
& FT-Transformer                                   & 0.486          & 0.476          & 0.472          & 0.478         \\
& FT-Transformer + \textsc{PTaRL}                  & 0.448          & 0.446          & 0.442          & 0.443         \\
\bottomrule
\end{tabular}}
\end{table}

R to Q4: 
We express our sincere gratitude for the insightful suggestions; they have proven immensely valuable in refining our paper. Classical methodologies, such as XGBoost, KNN, and SVM, enjoy widespread adoption among practitioners for solving tabular problems, owing to their commendable performance and user-friendly nature. The comparative analysis between deep learning models and traditional approaches is instrumental in advancing the overall model generality within the tabular domain. We hope that our proposed method could offer valuable insights into the augmentation of traditional methodologies.
